GATE: How to Keep Out Intrusive Neighbors

Graph Attention Networks (GATs) are designed to provide flexible neighborhood aggregation that assigns weights to neighbors according to their importance. In practice, however, GATs are often unable to switch off task-irrelevant neighborhood aggregation, as we show experimentally and analytically. To address this challenge, we propose GATE, a GAT extension that holds three major advantages: i) It alleviates over-smoothing by addressing its root cause of unnecessary neighborhood aggregation. ii) Similarly to perceptrons, it benefits from higher depth as it can still utilize additional layers for (non-)linear feature transformations in case of (nearly) switched-off neighborhood aggregation. iii) By down-weighting connections to unrelated neighbors, it often outperforms GATs on real-world heterophilic datasets. To further validate our claims, we construct a synthetic test bed to analyze a model's ability to utilize the appropriate amount of neighborhood aggregation, which could be of independent interest.

==> Tables/het_comparison.tex <==

\begin{tblr}{
  width = \linewidth,
  colspec = {Q[150]Q[160]Q[177]Q[154]Q[146]Q[146]},
  row{1} = {c},
  cell{2}{2} = {c},
  cell{2}{3} = {c},
  cell{2}{4} = {c},
  cell{2}{5} = {c},
  cell{2}{6} = {c},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{7}{2} = {c},
  cell{7}{3} = {c},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{8}{2} = {c},
  cell{8}{3} = {c},
  cell{8}{4} = {c},
  cell{8}{5} = {c},
  cell{8}{6} = {c},
  cell{9}{2} = {c},
  cell{9}{3} = {c},
  cell{9}{4} = {c},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{10}{2} = {c},
  cell{10}{3} = {c},
  cell{10}{4} = {c},
  cell{10}{5} = {c},
  cell{10}{6} = {c},
  cell{11}{2} = {c},
  cell{11}{3} = {c},
  cell{11}{4} = {c},
  cell{11}{5} = {c},
  cell{11}{6} = {c},
  cell{12}{2} = {c},
  cell{12}{3} = {c},
  cell{12}{4} = {c},
  cell{12}{5} = {c},
  cell{12}{6} = {c},
  cell{13}{2} = {c},
  cell{13}{3} = {c},
  cell{13}{4} = {c},
  cell{13}{5} = {c},
  cell{13}{6} = {c},
  cell{14}{2} = {c},
  cell{14}{3} = {c},
  cell{14}{4} = {c},
  cell{14}{5} = {c},
  cell{14}{6} = {c},
  cell{15}{2} = {c},
  cell{15}{3} = {c},
  cell{15}{4} = {c},
  cell{15}{5} = {c},
  cell{15}{6} = {c},
  cell{16}{2} = {c},
  cell{16}{3} = {c},
  cell{16}{4} = {c},
  cell{16}{5} = {c},
  cell{16}{6} = {c},
  cell{17}{2} = {c},
  cell{17}{3} = {c},
  cell{17}{4} = {c},
  cell{17}{5} = {c},
  cell{17}{6} = {c},
  cell{18}{2} = {c},
  cell{18}{3} = {c},
  cell{18}{4} = {c},
  cell{18}{5} = {c},
  cell{18}{6} = {c},
  cell{19}{2} = {c},
  cell{19}{3} = {c},
  cell{19}{4} = {c},
  cell{19}{5} = {c},
  cell{19}{6} = {c},
  cell{20}{2} = {c},
  cell{20}{3} = {c},
  cell{20}{4} = {c},
  cell{20}{5} = {c},
  cell{20}{6} = {c},
  hline{1,21} = {-}{0.08em},
  hline{2,4,6,10,18} = {-}{0.05em},
}
           & roman-empire & amazon-ratings & minesweeper  & tolokers     & questions    \\
GATE       & 89.51 $\pm$ 0.49 & 52.49 $\pm$ 0.46   & 92.82 $\pm$ 0.90 & \textbf{84.62 $\pm$ 0.69} & 78.46 $\pm$ 1.17 \\
GAT        & 80.87 $\pm$ 0.30 & 49.09 $\pm$ 0.63   & 92.01 $\pm$ 0.68 & 83.70 $\pm$ 0.47 & 77.43 $\pm$ 1.20 \\
GATE-Sep   & \textbf{89.78 $\pm$ 0.54} & \textbf{54.51 $\pm$ 0.38}   & \textbf{94.18 $\pm$ 0.43} & 84.48 $\pm$ 0.57 & 78.20 $\pm$ 1.00 \\
GAT-sep    & 88.75 $\pm$ 0.41 & 52.70 $\pm$ 0.62   & 93.91 $\pm$ 0.35 & 83.78 $\pm$ 0.43 & 76.79 $\pm$ 0.71 \\
GT         & 86.51 $\pm$ 0.73 & 51.17 $\pm$ 0.66   & 91.85 $\pm$ 0.76 & 83.23 $\pm$ 0.64 & 77.95 $\pm$ 0.68 \\
GT-sep     & 87.32 $\pm$ 0.39 & 52.18 $\pm$ 0.80   & 92.29 $\pm$ 0.47 & 82.52 $\pm$ 0.92 & 78.05 $\pm$ 0.93 \\
GCN        & 73.69 $\pm$ 0.74 & 48.70 $\pm$ 0.63   & 89.75 $\pm$ 0.52 & 83.64 $\pm$ 0.67 & 76.09 $\pm$ 1.27 \\
SAGE       & 85.74 $\pm$ 0.67 & 53.63 $\pm$ 0.39   & 93.51 $\pm$ 0.57 & 82.43 $\pm$ 0.44 & 76.44 $\pm$ 0.62 \\
H₂GCN      & 60.11 $\pm$ 0.52 & 36.47 $\pm$ 0.23   & 89.71 $\pm$ 0.31 & 73.35 $\pm$ 1.01 & 63.59 $\pm$ 1.46 \\
CPGNN      & 63.96 $\pm$ 0.62 & 39.79 $\pm$ 0.77   & 52.03 $\pm$ 5.46 & 73.36 $\pm$ 1.01 & 65.96 $\pm$ 1.95 \\
GPR-GNN    & 64.85 $\pm$ 0.27 & 44.88 $\pm$ 0.34   & 86.24 $\pm$ 0.61 & 72.94 $\pm$ 0.97 & 55.48 $\pm$ 0.91 \\
FSGNN      & 79.92 $\pm$ 0.56 & 52.74 $\pm$ 0.83   & 90.08 $\pm$ 0.70 & 82.76 $\pm$ 0.61 & \textbf{78.86 $\pm$ 0.92} \\
GloGNN     & 59.63 $\pm$ 0.69 & 36.89 $\pm$ 0.14   & 51.08 $\pm$ 1.23 & 73.39 $\pm$ 1.17 & 65.74 $\pm$ 1.19 \\
FAGCN      & 65.22 $\pm$ 0.56 & 44.12 $\pm$ 0.30   & 88.17 $\pm$ 0.73 & 77.75 $\pm$ 1.05 & 77.24 $\pm$ 1.26 \\
GBK-GNN    & 74.57 $\pm$ 0.47 & 45.98 $\pm$ 0.71   & 90.85 $\pm$ 0.58 & 81.01 $\pm$ 0.67 & 74.47 $\pm$ 0.86 \\
JacobiConv & 71.14 $\pm$ 0.42 & 43.55 $\pm$ 0.48   & 89.66 $\pm$ 0.40 & 68.66 $\pm$ 0.65 & 73.88 $\pm$ 1.16 \\
ResNet     & 65.88 $\pm$ 0.38 & 45.90 $\pm$ 0.52   & 50.89 $\pm$ 1.39 & 72.95 $\pm$ 1.06 & 70.34 $\pm$ 0.76 \\
ResNet+SGC & 73.90 $\pm$ 0.51 & 50.66 $\pm$ 0.48   & 70.88 $\pm$ 0.90 & 80.70 $\pm$ 0.97 & 75.81 $\pm$ 0.96 \\
ResNet+adj & 52.25 $\pm$ 0.40 & 51.83 $\pm$ 0.57   & 50.42 $\pm$ 0.83 & 78.78 $\pm$ 1.11 & 75.77 $\pm$ 1.24 
\end{tblr}

==> Tables/nbr-dep-syn-avg5runs.tex <==
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[73]Q[73]Q[179]Q[179]Q[179]Q[179]},
  cells = {c},
  cell{2}{1} = {r=3}{},
  cell{5}{1} = {r=3}{},
  cell{8}{1} = {r=3}{},
  hline{1,11} = {-}{0.08em},
  hline{2,5,8} = {-}{0.05em},
}
$k$ & $L$ & GAT$_S$ & GAT & GATE$_S$ & GATE\\
$1$ & $1$ & $93.60 \pm 1.26$ & $92.32 \pm 1.27$ & $\mathbf{96.40 \pm 0.70}$ & $93.52 \pm 1.27$\\
 & $2$ & $93.52 \pm 0.73$ & $92.72 \pm 2.69$ & $\mathbf{97.92 \pm 0.79}$ & $94.64 \pm 2.10$\\
 & $3$ & $88.16 \pm 4.86$ & $91.76 \pm 3.35$ & $92.08 \pm 4.59$ & $\mathbf{94.00 \pm 1.54}$\\
$2$ & $2$ & $90.40 \pm 1.30$ & $87.68 \pm 1.58$ & $\mathbf{93.84 \pm 0.51}$ & $88.72 \pm 2.50$\\
 & $3$ & $82.16 \pm 4.45$ & $88.88 \pm 2.12$ & $85.76 \pm 2.54$ & $\mathbf{93.44 \pm 3.27}$\\
 & $4$ & $84.00 \pm 5.00$ & $83.04 \pm 4.75$ & $\mathbf{89.20 \pm 2.33}$ & $87.76 \pm 2.36$\\
$3$ & $3$ & $84.32 \pm 3.18$ & $83.84 \pm 2.69$ & $87.52 \pm 1.82$ & $\mathbf{88.64 \pm 2.00}$\\
 & $4$ & $71.36 \pm 3.88$ & $75.92 \pm 7.63$ & $\mathbf{89.20 \pm 1.04}$ & $88.96 \pm 0.51$\\
 & $5$ & $80.16 \pm 4.75$ & $83.92 \pm 2.16$ & $86.08 \pm 0.79$ & $\mathbf{87.84 \pm 1.59}$
\end{tblr}

==> Tables/ogb-and-large-heterophily-datasets-gate-vs-gat.tex <==

\begin{tblr}{
  width = \linewidth,
  colspec = {Q[300]Q[165]Q[212]Q[238]},
  cells = {c},
  cell{3}{1} = {r=2}{},
  cell{8}{1} = {r=3}{},
  cell{11}{1} = {r=2}{},
  hline{1,13} = {-}{0.08em},
  hline{2-3,5-8,11} = {-}{0.05em},
}
Dataset & $L$ & GATE & GAT\\
minesweeper & $5$ & $\textbf{.676}$ & $.505$\\
tolokers & $5$ & $.638$ & $.638$\\
 & $10$ & $\textbf{.692}$ & $.616$\\
questions & $5$ & $\textbf{.643}$ & $.548$\\
roman-empire & $5$ & $\textbf{.759}$ & $.290$\\
amazon-ratings & $5$ & $.454$ & $\textbf{.459}$\\
ogb-arxiv & $3$ & $.773$ & $.719$*\\
 & $5$ & $.784$ & -\\
 & $8$ & $\textbf{.795}$ & -\\
ogb-products & $3$ & $.861$ & $.806$*\\
 & $5$ & $\textbf{.863}$ & -
\end{tblr}

==> Tables/table1.tex <==
\begin{table*}[h]
\centering
\caption{Self-sufficient learning: $S, C$ and $L$ denote graph structure, number of label classes, and number of network layers, respectively. Original (Orig.) and Randomized (Rand.) labels are used for the Cora structure. Most models achieve $100\%$ train accuracy, and entries marked with * refer to cases otherwise. GATE$_S$ also achieves $100\%$ train and test accuracy as GATE.}
\label{table:self-sufficient-learning}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[10]Q[10]Q[10]Q[150]Q[133]Q[131]Q[140]Q[133]Q[120]},
  row{even} = {c},
  row{5} = {c},
  row{7} = {c},
  row{11} = {c},
  row{13} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{c},
  cell{1}{3} = {r=2}{c},
  cell{1}{4} = {c=3}{0.41\linewidth,c},
  cell{1}{7} = {c=3}{0.4\linewidth,c},
  cell{3}{1} = {r=6}{},
  cell{3}{2} = {r=3}{c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{6}{2} = {r=3}{},
  cell{9}{1} = {r=6}{},
  cell{9}{2} = {r=3}{c},
  cell{9}{3} = {c},
  cell{9}{4} = {c},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{9}{7} = {c},
  cell{9}{8} = {c},
  cell{9}{9} = {c},
  cell{12}{2} = {r=3}{},
  hline{1,15} = {-}{0.08em},
  hline{2} = {4-9}{0.03em},
  hline{3,9} = {-}{0.05em},
  hline{6,12} = {2-9}{0.03em},
}
$S$                                       & $C$                                 & $L$ & Test Acc.(\%) @ Epoch of Min. Loss &                    &                      & Max Test Acc.(\%) @ Epoch &                    &                     \\
                                         &                                   &   & GAT$_S$                              & GAT                & GATE                 & GAT$_S$               & GAT                & GATE                \\
\begin{sideways}Cora\end{sideways}       & \begin{sideways}Orig.(7)\end{sideways} & 1 & \textbf{99.1@215}                  & 97.7@166         & 99.0@127           & 100@300             & 100@548          & \textbf{100@196}  \\
                                         &                                   & 2 & 93.4@218                           & 94.5@158         & \textbf{99.6@35}   & 94.4@187            & 94.6@156         & \textbf{100@40}   \\
                                         &                                   & 5 & 85.9@92                            & 85.5@72          & \textbf{98.4@36}   & 88@10               & 88.5@16          & \textbf{99.7@51}  \\
                                         & \begin{sideways}Rand.(7)\end{sideways} & 1 & 99.4@263                           & 99.8@268         & \textbf{100@104}   & 100@341             & 100@282          & \textbf{100@103}  \\
                                         &                                   & 2 & 61.7@2088*                         & 52.8@341*        & \textbf{99.9@36}   & 67.0@2221           & 57.0@125         & \textbf{100@38}   \\
                                         &                                   & 5 & 35.1@609                           & 32.1@1299        & \textbf{99.9@23}   & 37.4@327            & 36.7@12          & \textbf{100@42}   \\
\begin{sideways}ER ($p=0.01$)\end{sideways} & \begin{sideways}Rand.(2)\end{sideways} & 1 & 100@341                            & \textbf{100@182} & 100@1313           & 100@340             & \textbf{100@181} & 100@1304          \\
                                         &                                   & 2 & 99.2@100                           & 99.2@119         & \textbf{99.6@79}   & 100@114              & 100@301          & \textbf{100@80}   \\
                                         &                                   & 5 & 64.0@7778*                         & 99.6@239         & \textbf{100@45}    & 75.6@163            & 99.6@224         & \textbf{100@45}   \\
                                         & \begin{sideways}Rand.(8)\end{sideways} & 1 & 88.8@9578*                        & 98.4@3290        & \textbf{99.2@1755} & 90.4@9583           & 99.2@6727        & \textbf{100@2570} \\
                                         &                                   & 2 & 90.4@2459*                         & 94.8@2237        & \textbf{99.6@44}   & 94.8@1973*          & 97.6@6450        & \textbf{100@45}   \\
                                         &                                   & 5 & 23.6@8152                          & 26.0@8121        & \textbf{100@28}    & 36.0@255*           & 38.4@1011        & \textbf{100@27}   
\end{tblr}
\end{table*}
% \begin{tblr}{
%   width = \linewidth,
%   colspec = {Q[10]Q[10]Q[160]Q[148]Q[130]Q[148]Q[137]Q[129]},
%   cells = {c},
%   cell{1}{1} = {r=2}{},
%   cell{1}{2} = {r=2}{},
%   cell{1}{3} = {c=3}{0.448\linewidth},
%   cell{1}{6} = {c=3}{0.414\linewidth},
%   cell{3}{1} = {r=3}{},
%   cell{6}{1} = {r=3}{},
%   hline{1,9} = {-}{0.08em},
%   hline{2} = {3-8}{0.03em},
%   hline{3,6} = {-}{0.05em},
% }
% C                                 & L & Test Acc.(\%)@Epoch of Min. Train Loss &             &                    & Max Test Acc.(\%)@Epoch &            &                    \\
%                                   &   & GAT$_S$                              & GAT         & GATE               & GAT$_S$               & GAT        & GATE               \\
% \begin{sideways}O,7\end{sideways} & 1 & \textbf{99.1@215}                  & 97.7@166  & 99.0@127         & 100@300             & 100@548  & \textbf{100@196} \\
%                                   & 2 & 93.4@218                           & 94.5@158  & \textbf{99.6@35} & 94.4@187            & 94.6@156 & \textbf{100@40}  \\
%                                   & 5 & 85.9@92                            & 85.5@72   & \textbf{98.4@36} & 88@10               & 88.5@16  & \textbf{99.7@51} \\
% \begin{sideways}R,7\end{sideways} & 1 & 99.4@263                           & 99.8@268  & \textbf{100@104} & 100@341             & 100@282  & \textbf{100@103} \\
%                                   & 2 & 61.7@2088*                        & 52.8 @341* & \textbf{99.9@36} & 67.0@2221           & 57.0@125 & \textbf{100@38}  \\
%                                   & 5 & 35.1@609                           & 32.1@1299 & \textbf{99.9@23} & 37.4@327            & 36.7@12  & \textbf{100@42}  
% \end{tblr}

% \begin{tblr}{
%   width = \linewidth,
%   colspec = {Q[50]Q[50]Q[88]Q[206]Q[200]Q[206]Q[137]},
%   cells = {c},
%   cell{1}{1} = {r=2}{},
%   cell{1}{2} = {r=2}{},
%   cell{1}{3} = {r=2}{},
%   cell{1}{4} = {c=2}{0.406\linewidth},
%   cell{1}{6} = {c=2}{0.343\linewidth},
%   cell{3}{1} = {r=6}{},
%   cell{3}{2} = {r=3}{},
%   cell{6}{2} = {r=3}{},
%   cell{9}{1} = {r=6}{},
%   cell{9}{2} = {r=3}{},
%   cell{12}{2} = {r=3}{},
%   hline{1} = {-}{0.08em},
%   hline{2} = {4-7}{0.03em},
%   hline{3} = {-}{0.05em},
%   hline{6,9,12} = {2-7}{0.04em},
%   hline{15} = {2-7}{0.08em},
% }
% \begin{sideways}Structure\end{sideways}  & \begin{sideways}Labels ($C$)\end{sideways}   & \begin{sideways} Layers\end{sideways} & Test Acc.@Epoch of Min. Train Loss &                   & Max Test Acc.@Epoch &            \\
%                                          &                                            &                                      & GAT                                    & GATE              & GAT                   & GATE       \\
% \begin{sideways}Cora\end{sideways}       & \begin{sideways}Orig. (7)\end{sideways} & $1$                                  & 99.1@215                        & 99.0@127   & 100@300             & 100@196  \\
%                                          &                                            & $2$                                  & 93.4@218                        & 99.6@35    & 94.4@187            & 100@40   \\
%                                          &                                            & $5$                                  & 85.9@92                         & 98.4@36    & 88@10               & 99.7@51  \\
%                                          & \begin{sideways}Rand. (7)\end{sideways}    & $1$                                  & 99.4@263                        & 100@104    & 100@341             & 100@103  \\
%                                          &                                            & $2$                                  & 61.7@2088*                     & 99.9@36    & 67.0@2221           & 100@38   \\
%                                          &                                            & $5$                                  & 35.1@609                        & 99.9@23    & 37.4@327            & 100@42   \\
% \begin{sideways}ER($p=0.01$)\end{sideways} & \begin{sideways}Rand. (2)\end{sideways}   & $1$                                  & 100@341                         & 100@1313   & 100@340             & 100@1304\\ &                                            & $2$                                  & 99.2@100                        & 99.6@79    & 100@114              & 100@80   \\
%                                          &                                            & $5$                                  & 67.6@9751*                                      & 84.4@9858*                 & 81.2@1853                     & 87.6@7328          \\
%                                          & \begin{sideways}Rand. (8)\end{sideways}   & $1$                                  & 88.8@9578*                     & 99.2@1755  & 90.4@9583           & 100@2570 \\
%                                          &                                            & $2$                                  & 90.4@2459*                     & 99.6@44    & 94.8@1973    & 100@45   \\
%                                          &                                            & $5$                                  & 23.6@8152                       & 100@28     & 36.0@255     & 100@27   
% \end{tblr}
% \begin{tabular}{>{\centering\hspace{0pt}}m{0.05\linewidth}>{\centering\hspace{0pt}}m{0.05\linewidth}>{\centering\hspace{0pt}}m{0.083\linewidth}>{\centering\hspace{0pt}}m{0.233\linewidth}>{\centering\hspace{0pt}}m{0.196\linewidth}>{\centering\hspace{0pt}}m{0.173\linewidth}>{\centering\arraybackslash\hspace{0pt}}m{0.154\linewidth}} 
% \toprule
% \multirow{2}{0.05\linewidth}{\hspace{0pt}\Centering{}\rotcell{Struct.}} & \multirow{2}{0.05\linewidth}{\hspace{0pt}\Centering{}\rotcell{Labels}} & \multirow{2}{0.083\linewidth}{\hspace{0pt}\Centering{}\rotcell{Layers}} & \multicolumn{2}{>{\Centering\hspace{0pt}}m{0.429\linewidth}}{Test Acc. ($\%$) at \textasciitilde{}$0$ train loss~~@ Epoch} & \multicolumn{2}{>{\Centering\hspace{0pt}}m{0.326\linewidth}}{Max Test Acc. ($\%$)~@ Epoch} \\ 
% \cmidrule{4-7}
%  &  &  & GAT & GATE & GAT & GATE \\ 
% \midrule
% \multirow{6}{0.05\linewidth}{\hspace{0pt}\Centering{}\rotcell{Cora}} & \multirow{3}{0.05\linewidth}{\hspace{0pt}\Centering{}\rotcell{Original}} & $1$ & $99.1$@$215$ & $99$@$127$ & $100$@$300$ & $100$@$196$ \\
%  &  & $2$ & $93.4$@$218$ & $99.6$@$35$ & $94.4$@$187$ & $100$@$40$ \\
%  &  & $5$ & $85.9$@$92$ & $98.4$@$36$ & $88$@$10$ & $99.7$@$51$ \\ 
% \cmidrule{2-7}
%  & \multirow{3}{0.05\linewidth}{\hspace{0pt}\Centering{}\rotcell{Random}} & $1$ & $99.4$@$263$ & $100$@$104$ & $100$@$341$ & $100$@$103$ \\
%  &  & $2$ & $61.7$@$2088$\tablefootnote{Maximum train accuracy of $99.2\%$ achieved.} & $99.9$@$36$ & $67.0$@$2221$ & $100$@$38$ \\
%  &  & $5$ & $35.1$@$609$ & $99.9$@$23$ & $37.4$@$327$ & $100$@$42$ \\
% \bottomrule
% \end{tabular}
